The Double-Sided Silicon Strip Detector Tracker onboard the ComPair Balloon Flight

The ComPair balloon instrument is a prototype of the All-sky Medium Energy Gamma-ray Observatory (AMEGO) mission concept. AMEGO aims to bridge the spectral gap in sensitivity that currently exists from $\sim$100 keV to $\sim$100 MeV by being sensitive to both Compton and pair-production events. This is made possible through the use of four subsystems working together to reconstruct events: a double-sided silicon strip detector (DSSD) Tracker, a virtual Frisch grid cadmium zinc telluride (CZT) Low Energy Calorimeter, a ceasium iodide (CsI) High Energy Calorimeter, and an anti-coincidence detector (ACD) to reject charged particle backgrounds. Composed of 10 layers of DSSDs, ComPair's Tracker is designed to measure the position of photons that Compton scatter in the silicon, as well as reconstruct the tracks of electrons and positrons from pair-production as they propagate through the detector. By using these positions, as well as the absorbed energies in the Tracker and 2 Calorimeters, the energy and direction of the incident photon can be determined. This proceeding will present the development, testing, and calibration of the ComPair DSSD Tracker and early results from its balloon flight in August 2023.

==> extra.tex <==
The CZT and CsI calorimeters are calibrated similarly to the DSSD tracker. Radioactive sources with emission lines at higher energies that fall into the dynamic range of the two subsystems are used. Since the CZT calorimeter can measure up to 10 MeV, and the CsI calorimeter can measure energies $>$ 20 MeV, sources such as Na-22, Cs-137, and Th-228 are used.


In order to do this, a large cross section for these interactions is required, which necessitates the need for a low Z material. Additionally, the detectors must be able to measure the secondary electrons and positrons accurately. Historically, both Germanium (Ge) and Silicon (Si) detectors have been used for this. In \textit{ComPair}, Si detectors are preferred over Ge detectors because: 1) Si detectors provide better angular resolution compared to Ge detectors (Fig.~\ref{fig:SivsGe}) and, 2) Ge detectors can be very expensive and need reduced temperatures in order to be used, which would add a lot of passive material and weight due to the necessary coolers.

\begin{figure}[H]
\centering
    \includegraphics[width=100mm]{SivsGe.png}
\caption{Plot of angular resolution vs the atomic number Z of identical detectors \cite{Zoglauer_2006}}
\label{fig:SivsGe}
\end{figure}

Due to the detector's electronics, as well as defects in the silicon, charges can be picked up on the electrodes of the detector which set a lower limit on what signal the tracker can see. This is effectively the detector's baseline noise. For this reason, a limit is set for how much charge is required to be seen as a signal (real event), called the triggering threshold.

(Left) Heat map of layer 1 generated from a Sr-90 source placed directly on top of the detector. Sr-90 is used because it is a beta source, therefore it emits electrons which interact more quickly in matter compared to photons of the equivalent energy. This leads to the source producing a more intense radiation hot spot near the emission region, allowing for a quick check of the detector's position resolution. (Right) Heat map of layer 1 generated from a Na-22 source placed above the detector. Since it is a gamma source, it's able to illuminate the entire detector. This allows us to quickly see any strips that are unresponsive (the black lines).
